On Estimating the Perimeter Using the Alpha-Shape

We consider the problem of estimating the perimeter of a smooth domain in the plane based on a sample from the uniform distribution over the domain. We study the performance of the estimator defined as the perimeter of the alpha-shape of the sample. Some numerical experiments corroborate our theoretical findings.

==> codes-figures/2-ball.tex <==
\begin{center}
\psset{unit=1cm}

\begin{pspicture}(5,5.618034)%\psgrid(0,0)(20,13)
\pscircle(1.5,4.118034){1.5}
\psdot(1.5,4.118034)
\pscircle(3.5,4.118034){1.5}
\psdot(3.5,4.118034)
\pscircle(2.5,1.5){1.5}
\uput[135](0.3,5.2){$B$}
\uput[45](4.7,5.2){$B'$}
\uput[270](3.7,0.2){$B_0$}
\uput[30](2.5,3){$x$}
\psdot(2.5,3)
\psline{<->}(1.5,4.118034)(3.5,4.118034)
\uput[90](2.5,4.118034){$d$}
\psline{<->}(2.5,4.118034)(2.5,3)
\uput[0](2.5,3.559017){$h$}
\psdot(2.5,1.5)
\psline{<->}(2.5,1.5)(1.5,4.118034)
\psline{<->}(2.5,1.5)(2.5,3)
\uput[0](2.5,2.25){$\alpha$}

%\uput[90](2.216312, 2.36574){$x_2$}
% \psdot(1.505025,2.194975)
% \uput[90](1.505025,2.194975){$x_1$}
% \psline(1.505025,2.194975)(2.216312, 2.36574)
%\uput[135](2,2.4){$x^{*}$}
%\uput[225](2,1.7){$z$}
%\uput[45](2,2){$y$}
%\uput[45](2,0){$B^{-}$}
\end{pspicture}
\end{center}

==> codes-figures/disc.tex <==

\begin{center}
\psset{unit=2.5cm}
\begin{pspicture}(2,2)%\psgrid(0,0)(20,13)
\pscircle(1,1){1}
\pscircle(1,1){0.25}
%\pcline{|-|}(1,1.25)(1,1)
%\aput{:U}{\scriptsize $r=0.25$}
%\psline{<->}(1,1.25)(1,1)
%\uput[0](1,1){$r=0.25$}
\end{pspicture}
\end{center}

==> perimeter-figures/alphahull/R/alphahull <==
.First.lib <- function(libname, pkgname)
{
    fullName <- paste("package", pkgname, sep=":")
    myEnv <- as.environment(match(fullName, search()))
    barepackage <- sub("([^-]+)_.*", "\\1", pkgname)
    dbbase <- file.path(libname, pkgname, "R", barepackage)
    rm(.First.lib, envir = myEnv)
    lazyLoad(dbbase, myEnv)
    if(exists(".First.lib", envir = myEnv, inherits = FALSE)) {
        f <- get(".First.lib", envir = myEnv, inherits = FALSE)
        if(is.function(f))
            f(libname, pkgname)
        else
            stop(gettextf("package '%s' has a non-function '.First.lib'",
                          pkgname),
                 domain = NA)
    }
}

